Optical Variability Properties of Southern TESS Blazars

We present a study of high-cadence, high-precision, optical light curves from the TESS satellite of 67 blazars in the southern sky. We provide descriptive flux statistics, power spectral density model parameters, and characteristic variability timescales. We find that only 15 BL Lacertae objects (BLLs) and 18 Flat Spectrum Radio Quasars (FSRQs) from the initial 26 and 41, respectively exhibit statistically-significant variability. We employ an adapted Power Spectral Response method to test the goodness of fit for the power spectral density function (PSD) to 3 power-law variant models. From our best-fitting description of the PSD, we extract the high-frequency power-spectral slopes and, if present, determine the significant bend or break in the model to identify characteristic timescales. We find no significant difference in the excess variance or rms-scatter between blazar subpopulations. We identify a linear rms-flux relation in ~69% of our sample, in which ~20% show a strong correlation. We find that both subpopulations of blazars show power spectral slope of $\alpha$~2 in which a broken power-law best fits 5 BLL & 6 FSRQ and a bending power-law best fits 1 BLL & 5 FSRQ. The shortest timescales of variability in each light curve range widely from minutes to weeks. Additionally, the objects' characteristic timescales range from ~0.8-8 days, consistent with the optical variability originating in the jet.

==> acknowledgements.tex <==
\label{sec:acknowledgements}

\begin{acknowledgments}
    Funding for this work was provided by the SMU Moody School of Graduate \& Advanced Studies, and, NASA grant 80NSSC22K0741. Special thanks to those who provided additional insight/development in the beta-testing of \texttt{quaver}, particularly Ethan Poore, for testing the reliability of \texttt{quaver} regressions to other methodologies. Additional gratitude goes to Dr. Michael Carini for providing valuable insight into the physical interpretation of our results. This paper includes data collected with the TESS mission, obtained from the MAST data archive at the Space Telescope Science Institute (STScI) all of which can be found at DOI:\dataset[10.17909/rar9-cn43]{https://doi.org/10.17909/rar9-cn43}. Funding for the TESS mission is provided by the NASA Explorer Program. STScI is operated by the Association of Universities for Research in Astronomy, Inc., under NASA contract NAS 5–26555. Additionally, this research has made use of the SIMBAD database, operated at CDS, Strasbourg, France, as well as data from the European Space Agency (ESA) mission Gaia (\url{https://www.cosmos.esa.int/gaia}), processed by the Gaia Data Processing and Analysis Consortium (DPAC, \url{https://www.cosmos.esa.int/web/gaia/dpac/consortium}) \citep{irsa2019} as well as \citet{NED2019}, which is funded by the National Aeronautics and Space Administration and operated by the California Institute of Technology. Funding for the DPAC has been provided by national institutions, in particular, the institutions participating in the Gaia Multilateral Agreement. Software packages which were made use of in this work include Lightkurve, a Python package for Kepler and TESS data analysis \citep{lightkurve2018}; Astropy:9 a community-developed core Python package and an ecosystem of tools and resources for astronomy \citep{astropy:2022}; and astroquery, an astronomical web-querying package in Python \citep{Ginsburg2019b}). We also gratefully acknowledge comments from an anonymous referee which improved the clarity and quality of the manuscript.
    
    \software{Astrocut \citep{Brasseur2019}, Astropy \citep{astropy:2013, astropy:2018, astropy:2022}, Astroquery \citep{Ginsburg2019b} quaver \citep{Smith2023}, \& Lightkurve \citep{lightkurve2018}} 
\end{acknowledgments}
